Towards Low-Latency Event-based Obstacle Avoidance on a FPGA-Drone

This work quantitatively evaluates the performance of event-based vision systems (EVS) against conventional RGB-based models for action prediction in collision avoidance on an FPGA accelerator. Our experiments demonstrate that the EVS model achieves a significantly higher effective frame rate (1 kHz) and lower temporal (-20 ms) and spatial prediction errors (-20 mm) compared to the RGB-based model, particularly when tested on out-of-distribution data. The EVS model also exhibits superior robustness in selecting optimal evasion maneuvers. In particular, in distinguishing between movement and stationary states, it achieves a 59 percentage point advantage in precision (78% vs. 19%) and a substantially higher F1 score (0.73 vs. 0.06), highlighting the susceptibility of the RGB model to overfitting. Further analysis in different combinations of spatial classes confirms the consistent performance of the EVS model in both test data sets. Finally, we evaluated the system end-to-end and achieved a latency of approximately 2.14 ms, with event aggregation (1 ms) and inference on the processing unit (0.94 ms) accounting for the largest components. These results underscore the advantages of event-based vision for real-time collision avoidance and demonstrate its potential for deployment in resource-constrained environments.

==> sec/6_hardware.tex <==
\section{Real-World Evaluation}
\label{sec:eval}

\subsection{Hardware Implementation}
We integrate the presented prediction framework on the SwiftEagle's \cite{vogt2024IROS} onboard \ac{SoC} by a hardware-software co-design approach, depicted in \Cref{fig:hardware_design}. On the programmable hardware part realized with the \ac{FPGA} fabric, both, the custom optimized \ac{EVS} frame aggregation, as well as the commercial inference module (AMD Xilinx \ac{DPU}) are located. The software part is split into two main components: orchestration of the inference and reaction to the inference results. The orchestration is handled by a custom application the on-board quad-core ARM Cortex A52 processors running Yocto\footnote{\url{https://github.com/Xilinx/meta-xilinx}} Linux (APU). Finally, evaluation of the inference results and taking appropriate action is handled by the on-board microcontroller (ARM R5, RPU), which also runs the SwiftEagle flight stack.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{media/dpu_architecture.pdf}
    \caption{\textbf{Hardware/Software Co-design approach} integrating the detection network on the SwiftEagle platform}
    \label{fig:hardware_design}
\end{figure}

The frame aggregation on the programmable logic, processes raw \ac{EVS} events directly, and accumulates them in 80x80 pixel frames with fully configurable accumulation time. Aggregated \ac{EVS} frames are then normalized and transferred to the DDR memory upon completion. To prevent loss of events during the data transfer from fabric to DDR, we implemented a double-buffering scheme on the fabric: while one buffer is transferred to DDR, the other buffer is used for aggregation, and vice versa. The  \ac{DPU} is configured as such: type \emph{dpuczdx8g}, with architecture \emph{1600} and 1 core. The \ac{DPU} can directly read the accumulated frames from DDR memory and also stores the inference outputs again in \ac{DDR} memory. 

On the software side, the custom developed application receives a hardware trigger when a new \ac{EVS} frame is available in the DDR memory and reacts by triggering the \ac{DPU} to run an inference. The application also ensures setup of the \ac{DPU} with the model, as well as assigning correct memory addresses for frames and inference results. This approach allows the usage of the tool-chain provided by the \ac{DPU} manufacturer AMD. The Firmware of the on-board microcontroller finally implements the decision logic for evasion decision.

\subsection{Real-World Results}

\textcolor{red}{also show shorter integration time}
The implemented hardware/software co-design with it's worst case end-to-end latency depicted in \Cref{fig:hardware_latency}. The \ac{EVS} latency was estimated in \cite{vogt2024IROS} and \cite{gallego_event-based_2022} to be approx. \qty{170}{\micro\second}, the decoding of the CSI2 MIPI data stream from the \ac{EVS} takes below \qty{40}{\micro\second}. Afterwards the events are decoded and aggregated with a variable integration time. This is the part with largest latency, as \qty{20}{\milli\second} were chosen for this step. Once the aggregation is complete, the write to DDR memory and signaling the APU requires approx. \qty{90}{\micro\second}, the inference runs within \qty{0.94}{\milli\second} on the FPGA accelerator. Finally the RPU is signaled to read the inference results and decides with a simple decision tree which action execute on the flight controller.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{media/latency.png}
    \caption{\textbf{End-to-end latency} split into the individual compute parts, including all data movements from EVS to final decision on the RPU.}
    \label{fig:hardware_latency}
\end{figure}

With the system latency characterized, we expanded the dataset by additional 32 ball throws where the input- as well as output tensors to the \ac{DPU} were recorded, to ensure proper operation in a real-world environment. 


